Expected Possession Value of Control and Duel Actions for Soccer Player's Skills Estimation

Estimation of football players' skills is one of the key tasks in sports analytics. This paper introduces multiple extensions to a widely used model, expected possession value (EPV), to address some key challenges such as selection problem. First, we assign greater weights to events occurring immediately prior to the shot rather than those preceding them (decay effect). Second, our model incorporates possession risk more accurately by considering the decay effect and effective playing time. Third, we integrate the assessment of individual player ability to win aerial and ground duels. Using the extended EPV model, we predict this metric for various football players for the upcoming season, particularly taking into account the strength of their opponents.

==> tables/PCR_predictionsBocaJuniors.tex <==
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
    \# & player & team & age & PCR & PCR\_pred & PCR\_adj & stay\_proba \\ \hline
    1 & J. Doku & Manchester City & 21.2 & 0.299 & 0.168 & 0.174 & 0.961 \\ \hline
    2 & O. Dembélé & PSG & 26.3 & 0.215 & 0.17 & 0.17 & 0.868 \\ \hline
    3 & Vinícius Júnior & Real Madrid & 23.1 & 0.136 & 0.155 & 0.157 & 0.938 \\ \hline
    4 & K. Kvaratskhelia & Napoli & 22.5 & 0.195 & 0.148 & 0.152 & 0.954 \\ \hline
    5 & O. Sahraoui & Heerenveen & 22.2 & 0.151 & 0.153 & 0.151 & 0.882 \\ \hline
    6 & Sávio & Girona & 19.4 & 0.174 & 0.146 & 0.15 & 0.96 \\ \hline
    7 & Haissem Hassan & Sporting Gijon & 21.5 & 0.125 & 0.153 & 0.148 & 0.873 \\ \hline
    8 & Bryan Zaragoza & Granada & 21.9 & 0.162 & 0.145 & 0.148 & 0.961 \\ \hline
    9 & E. Zhegrova & Lille & 24.4 & 0.097 & 0.146 & 0.147 & 0.907 \\ \hline
    10 & M. Olise & Crystal Palace & 21.7 & 0.182 & 0.145 & 0.146 & 0.862 \\ \hline
    11 & Á. Di María & Benfica Portugal & 35.5 & 0.207 & 0.157 & 0.145 & 0.578 \\ \hline
    12 & N. Lang & PSV & 24.2 & 0.196 & 0.151 & 0.144 & 0.74 \\ \hline
    13 & Francisco Conceicão & Porto & 20.7 & 0.233 & 0.145 & 0.144 & 0.905 \\ \hline
    14 & Nico Williams & Athletic Bilbao & 21.1 & 0.199 & 0.139 & 0.142 & 0.956 \\ \hline
    15 & M. Politano & Napoli & 30.1 & 0.188 & 0.143 & 0.142 & 0.796 \\ \hline
    16 & J. Dompé & Hamburger SV & 28.0 & 0.158 & 0.149 & 0.142 & 0.768 \\ \hline
    17 & David Neres & Benfica Portugal & 26.5 & 0.25 & 0.149 & 0.142 & 0.708 \\ \hline
    18 & J. Clarke & Sunderland & 22.7 & 0.268 & 0.143 & 0.141 & 0.939 \\ \hline
    19 & T. Ali & Malmo FF & 24.8 & 0.277 & 0.144 & 0.14 & 0.828 \\ \hline
    20 & Pedro Neto & Wolverhampton & 23.4 & 0.131 & 0.138 & 0.139 & 0.855 \\ \hline
    21 & Daniel Podence & Olympiacos Piraeus & 27.8 & 0.252 & 0.143 & 0.137 & 0.8 \\ \hline
    22 & Rafael Leão & Milan & 24.2 & 0.178 & 0.135 & 0.137 & 0.913 \\ \hline
    23 & K. Coman & Bayern Munchen & 27.2 & 0.095 & 0.135 & 0.136 & 0.861 \\ \hline
    24 & B. Gruda & Mainz 05 & 19.2 & 0.163 & 0.135 & 0.135 & 0.823 \\ \hline
    25 & T. Corbeanu & Grasshopper & 21.2 & 0.152 & 0.136 & 0.134 & 0.869 \\ \hline
    26 & R. Sterling & Chelsea & 28.7 & 0.152 & 0.133 & 0.134 & 0.828 \\ \hline
    27 & F. Reese & Hertha BSC & 25.7 & 0.2 & 0.137 & 0.133 & 0.861 \\ \hline
    28 & J. Bakayoko & PSV & 20.3 & 0.194 & 0.133 & 0.132 & 0.928 \\ \hline
    29 & C. Ejuke & Antwerp & 25.6 & 0.158 & 0.134 & 0.132 & 0.848 \\ \hline
    30 & M. Edwards & Sporting CP & 24.7 & 0.277 & 0.134 & 0.131 & 0.866 \\ \hline
    31 & E. Soares & Trencin & 24.8 & 0.098 & 0.136 & 0.131 & 0.869 \\ \hline
    32 & R. Sottil & Fiorentina & 24.2 & 0.097 & 0.13 & 0.13 & 0.84 \\ \hline
    33 & S. Villa & Boca Juniors & 26.7 & 0.109 & 0.133 & 0.13 & 0.89 \\ \hline
    34 & J. Boga & Nice & 26.6 & 0.079 & 0.129 & 0.13 & 0.894 \\ \hline
    35 & Y. Soteldo & Santos & 25.8 & 0.27 & 0.144 & 0.13 & 0.485 \\ \hline
    36 & Milson & Maccabi Tel Aviv & 23.9 & 0.178 & 0.133 & 0.129 & 0.856 \\ \hline
    37 & A. Mitriță & Universitatea Craiova & 28.4 & 0.195 & 0.129 & 0.127 & 0.906 \\ \hline
    38 & H. Ziyech & Galatasaray & 30.4 & 0.166 & 0.14 & 0.127 & 0.481 \\ \hline
    39 & K. Mitoma & Brighton & 26.2 & 0.215 & 0.125 & 0.127 & 0.856 \\ \hline
    40 & J. Sancho & Borussia Dortmund & 23.4 & 0.224 & 0.126 & 0.126 & 0.858 \\ \hline
    41 & T. Kubo & Real Sociedad & 22.2 & 0.162 & 0.124 & 0.126 & 0.933 \\ \hline
    42 & C. Hudson-Odoi & Nottingham Forest & 22.8 & 0.114 & 0.124 & 0.126 & 0.884 \\ \hline
    43 & M. Simon & Nantes & 28.1 & 0.125 & 0.127 & 0.125 & 0.801 \\ \hline
    44 & F. Chiesa & Juventus & 25.8 & 0.195 & 0.122 & 0.125 & 0.932 \\ \hline
    45 & I. Akhomach & Villarreal & 19.3 & 0.094 & 0.122 & 0.124 & 0.936 \\ \hline
    46 & R. Cherki & Olympique Lyonnais & 20.0 & 0.052 & 0.124 & 0.124 & 0.905 \\ \hline
    47 & T. Alexander-Arnold & Liverpool & 24.9 & 0.113 & 0.122 & 0.124 & 0.878 \\ \hline
    48 & Ângelo Gabriel & Strasbourg & 18.6 & 0.125 & 0.122 & 0.123 & 0.918 \\ \hline
    49 & Dudu & Palmeiras & 31.3 & 0.172 & 0.134 & 0.123 & 0.57 \\ \hline
    50 & K. Grosicki & Pogon Szczecin & 35.1 & 0.155 & 0.135 & 0.123 & 0.508 \\ \hline
\end{tabular}


==> tables/PCR_predictionsFlamengo.tex <==
\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|l|l|l|l|l|l|l|}
    \hline
        \# & player & team & age & PCR & PCR\_pred & PCR\_adj & stay\_proba \\ \hline
        1 & O. Dembélé & PSG & 26.3 & 0.215 & 0.169 & 0.167 & 0.868 \\ \hline
        2 & J. Doku & Manchester City & 21.2 & 0.299 & 0.163 & 0.166 & 0.961 \\ \hline
        3 & Vinícius Júnior & Real Madrid & 23.1 & 0.136 & 0.149 & 0.15 & 0.938 \\ \hline
        4 & O. Sahraoui & Heerenveen & 22.2 & 0.151 & 0.148 & 0.144 & 0.882 \\ \hline
        5 & Á. Di María & Benfica Portugal & 35.5 & 0.207 & 0.157 & 0.144 & 0.578 \\ \hline
        6 & K. Kvaratskhelia & Napoli & 22.5 & 0.195 & 0.139 & 0.141 & 0.954 \\ \hline
        7 & T. Ali & Malmo FF & 24.8 & 0.277 & 0.147 & 0.141 & 0.828 \\ \hline
        8 & Francisco Conceicão & Porto & 20.7 & 0.233 & 0.143 & 0.141 & 0.905 \\ \hline
        9 & Sávio & Girona & 19.4 & 0.174 & 0.139 & 0.14 & 0.96 \\ \hline
        10 & M. Olise & Crystal Palace & 21.7 & 0.182 & 0.139 & 0.139 & 0.862 \\ \hline
        11 & N. Lang & PSV & 24.2 & 0.196 & 0.147 & 0.138 & 0.74 \\ \hline
        12 & Bryan Zaragoza & Granada & 21.9 & 0.162 & 0.135 & 0.136 & 0.961 \\ \hline
        13 & E. Zhegrova & Lille & 24.4 & 0.097 & 0.136 & 0.136 & 0.907 \\ \hline
        14 & T. Corbeanu & Grasshopper & 21.2 & 0.152 & 0.139 & 0.136 & 0.869 \\ \hline
        15 & Nico Williams & Athletic Bilbao & 21.1 & 0.199 & 0.133 & 0.135 & 0.956 \\ \hline
        16 & Haissem Hassan & Sporting Gijon & 21.5 & 0.125 & 0.138 & 0.133 & 0.873 \\ \hline
        17 & David Neres & Benfica Portugal & 26.5 & 0.25 & 0.141 & 0.133 & 0.708 \\ \hline
        18 & M. Edwards & Sporting CP & 24.7 & 0.277 & 0.134 & 0.131 & 0.866 \\ \hline
        19 & J. Dompé & Hamburger SV & 28.0 & 0.158 & 0.138 & 0.13 & 0.768 \\ \hline
        20 & M. Politano & Napoli & 30.1 & 0.188 & 0.132 & 0.129 & 0.796 \\ \hline
        21 & K. Coman & Bayern Munchen & 27.2 & 0.095 & 0.129 & 0.128 & 0.861 \\ \hline
        22 & C. Ejuke & Antwerp & 25.6 & 0.158 & 0.131 & 0.127 & 0.848 \\ \hline
        23 & Y. Soteldo & Santos & 25.8 & 0.27 & 0.143 & 0.127 & 0.485 \\ \hline
        24 & Rafael Leão & Milan & 24.2 & 0.178 & 0.126 & 0.126 & 0.913 \\ \hline
        25 & R. Sterling & Chelsea & 28.7 & 0.152 & 0.126 & 0.125 & 0.828 \\ \hline
        26 & Pedro Neto & Wolverhampton & 23.4 & 0.131 & 0.125 & 0.125 & 0.855 \\ \hline
        27 & B. Gruda & Mainz 05 & 19.2 & 0.163 & 0.125 & 0.124 & 0.823 \\ \hline
        28 & J. Bakayoko & PSV & 20.3 & 0.194 & 0.125 & 0.123 & 0.928 \\ \hline
        29 & J. Boga & Nice & 26.6 & 0.079 & 0.124 & 0.123 & 0.894 \\ \hline
        30 & Daniel Podence & Olympiacos Piraeus & 27.8 & 0.252 & 0.128 & 0.122 & 0.8 \\ \hline
        31 & R. Sottil & Fiorentina & 24.2 & 0.097 & 0.123 & 0.121 & 0.84 \\ \hline
        32 & M. Simon & Nantes & 28.1 & 0.125 & 0.123 & 0.12 & 0.801 \\ \hline
        33 & F. Reese & Hertha BSC & 25.7 & 0.2 & 0.124 & 0.12 & 0.861 \\ \hline
        34 & A. Skov Olsen & Club Brugge & 23.6 & 0.147 & 0.12 & 0.119 & 0.917 \\ \hline
        35 & J. Clarke & Sunderland & 22.7 & 0.268 & 0.121 & 0.118 & 0.939 \\ \hline
        36 & Milson & Maccabi Tel Aviv & 23.9 & 0.178 & 0.122 & 0.117 & 0.856 \\ \hline
        37 & T. Kubo & Real Sociedad & 22.2 & 0.162 & 0.117 & 0.117 & 0.933 \\ \hline
        38 & Dudu & Palmeiras & 31.3 & 0.172 & 0.129 & 0.117 & 0.57 \\ \hline
        39 & Serginho & Viborg & 22.5 & 0.182 & 0.124 & 0.117 & 0.719 \\ \hline
        40 & R. Cherki & Olympique Lyonnais & 20.0 & 0.052 & 0.118 & 0.117 & 0.905 \\ \hline
        41 & F. Chiesa & Juventus & 25.8 & 0.195 & 0.116 & 0.117 & 0.932 \\ \hline
        42 & M. Solomon & Tottenham Hotspur & 24.1 & 0.27 & 0.12 & 0.116 & 0.714 \\ \hline
        43 & K. Grosicki & Pogon Szczecin & 35.1 & 0.155 & 0.129 & 0.116 & 0.508 \\ \hline
        44 & J. Sancho & Borussia Dortmund & 23.4 & 0.224 & 0.117 & 0.116 & 0.858 \\ \hline
        45 & H. Ziyech & Galatasaray & 30.4 & 0.166 & 0.129 & 0.116 & 0.481 \\ \hline
        46 & A. Mitriță & Universitatea Craiova & 28.4 & 0.195 & 0.119 & 0.116 & 0.906 \\ \hline
        47 & O. Niang & Riga & 21.4 & 0.296 & 0.126 & 0.116 & 0.734 \\ \hline
        48 & A. Nusa & Club Brugge & 18.3 & 0.143 & 0.118 & 0.115 & 0.872 \\ \hline
        49 & K. Mitoma & Brighton & 26.2 & 0.215 & 0.116 & 0.115 & 0.856 \\ \hline
        50 & Ângelo Gabriel & Strasbourg & 18.6 & 0.125 & 0.116 & 0.115 & 0.918 \\ \hline
    \end{tabular}
\end{table}
